Execution-based Code Generation using Deep Reinforcement Learning

The utilization of programming language (PL) models, pre-trained on large-scale code corpora, as a means of automating software engineering processes has demonstrated considerable potential in streamlining various code generation tasks such as code completion, code translation, and program synthesis. However, current approaches mainly rely on supervised fine-tuning objectives borrowed from text generation, neglecting unique sequence-level characteristics of code, including but not limited to compilability as well as syntactic and functional correctness. To address this limitation, we propose PPOCoder, a new framework for code generation that synergistically combines pre-trained PL models with Proximal Policy Optimization (PPO) which is a widely used deep reinforcement learning technique. By utilizing non-differentiable feedback from code execution and structure alignment, PPOCoder seamlessly integrates external code-specific knowledge into the model optimization process. It's important to note that PPOCoder is a task-agnostic and model-agnostic framework that can be used across different code generation tasks and PLs. Extensive experiments on three code generation tasks demonstrate the effectiveness of our proposed approach compared to SOTA methods, achieving significant improvements in compilation success rates and functional correctness across different PLs.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables_figs_tex/ablation_fig_1.tex <==
% \begin{figure*}[!ht]
% \centering
% %\includegraphics[width=0.48\textwidth]{whole model.png}
% \includegraphics[width=0.7\linewidth]{figures/ablation1.png}
% \caption{Ablation study experiments on Java-Python translation with different configurations of (a) reward, and (b) loss 
% }
% \label{fig:ablation1}
% \end{figure*}


\begin{figure}[t]
\centering
%\includegraphics[width=0.48\textwidth]{whole model.png}
\includegraphics[width=\linewidth]{figures/ablation_all1_v5.jpg}
\caption{
% \vspace{-0.5em}
Ablation experiment results on code translation with different configurations of (a) reward, and (b) loss
% , (c) action space size, and (d) number of synthetic samples. 
\vspace{-1.0em}
}
\label{fig:ablation1}
\end{figure}


% \begin{figure*}[!ht]
% \centering
% %\includegraphics[width=0.48\textwidth]{whole model.png}
% \includegraphics[width=\linewidth]{figures/ablation_all2.jpg}
% \caption{Ablation study experiments on Java-Python translation with different configurations of (a) reward, and (b) loss 
% }
% \label{fig:ablation1}
% \end{figure*}

==> tables_figs_tex/ablation_fig_2.tex <==
\begin{figure*}[!ht]
\centering
%\includegraphics[width=0.48\textwidth]{whole model.png}
\includegraphics[width=0.7\linewidth]{figures/ablation2.png}
\caption{Ablation study on Python-C\# translation with different variants of (a) action space size, and (b) number of synthetic samples.  
}
\label{fig:ablation2}
\end{figure*}

==> tables_figs_tex/case_study_cpp_python.tex <==
\begin{table*}[h!]
% \hskip-0.5cm
\caption{Qualitative comparison for C++-Python translation between CodeT5 and \modelname. i) CodeT5 generates an extra closing parenthesis. ii) CodeT5 generates the wrong syntax for function declaration, \modelname is able to generate the correct Python syntax using \begin{tt}def\end{tt} keyword.}
\label{tab:cpp_python_qualitative}
\begin{tabular}{|P{5.0cm}|P{5.0cm}|P{5.0cm}|}

\cline{2-3}\multicolumn{1}{c}{}             & \multicolumn{2}{|c|}{\normalsize{\textbf{Translated Python}}}\\
\hline
\normalsize{\textbf{Source C++}} & \normalsize{\textbf{CodeT5}} & \normalsize{\textbf{\modelname}}\\
\hline
\begin{lstlisting}[style=C++]
#include <bits/stdc++.h>
using namespace std ;
int func ( int N , int P ) {
  int sumUptoN = ( N * ( N + 1 ) / 2 ) ;
  int sumOfMultiplesOfP ;
  if ( N < P ) {
    return sumUptoN ;
  }
  else if ( ( N / P ) == 1 ) {
    return sumUptoN - P + 1 ;
  }
  sumOfMultiplesOfP = ( ( N / P ) * ( 2 * P + ( N / P - 1 ) * P ) ) / 2 ;
  return ( sumUptoN + func ( N / P , P ) - sumOfMultiplesOfP ) ;
}
int main ( ) {
  int N = 10 , P = 5 ;
  cout << func ( N , P ) << "
  " ;
  return 0 ;
}

\end{lstlisting} &
\begin{lstlisting}[style=py]
def func ( N , P ) :
    sumUptoN = ( N * ( N + 1 ) // 2 )
    sumOfMultiplesOfP = 0
    if ( N < P ) :
        return sumUptoN
    elif ( ( N / P ) == 1 ) :
        return sumUptoN - P + 1
    sumOfMultiplesOfP = ( ( N / P ) * ( 2 * P + ( N / P - 1 ) * P ) ) <@\textcolor{red}{// 2 )}@>
    return ( sumUptoN + func ( N // P , P ) - sumOfMultiplesOfP )
N = 10
P = 5
print ( func ( N , P ) )
\end{lstlisting}&
\begin{lstlisting}[style=py]
def func ( N , P ) :
    sumUptoN = int ( N * ( N + 1 ) / 2 )
    sumOfMultiplesOfP = 0
    if ( N < P ) :
        return sumUptoN
    elif ( ( N / P ) == 1 ) :
        return sumUptoN - P + 1
    sumOfMultiplesOfP = ( ( N / P ) * ( 2 * P + ( N / P - 1 ) * P ) ) <@\textcolor{blue}{// 2}@>
    return ( sumUptoN + func ( N // P , P ) - sumOfMultiplesOfP )
if __name__ == '__main__' :
    N = 10
    P = 5
    print ( func ( N , P ) )
\end{lstlisting}\\
\hline
\begin{lstlisting}[style=C++]
#include <bits/stdc++.h>
using namespace std ;
int findWays ( int N , int dp [ ] ) {
  if ( N == 0 ) {
    return 1 ;
  }
  if ( dp [ N ] != -1 ) {
    return dp [ N ] ;
  }
  int cnt = 0 ;
  for ( int i = 1 ;
  i <= 6 ;
  i ++ ) {
    if ( N - i >= 0 ) {
      cnt = cnt + findWays ( N - i , dp ) ;
    }
  }
  return dp [ N ] = cnt ;
}
int main ( ) {
  int N = 4 ;
  int dp [ N + 1 ] ;
  memset ( dp , -1 , sizeof ( dp ) ) ;
  cout << findWays ( N , dp ) ;
  return 0 ;
}
\end{lstlisting} &
\begin{lstlisting}[style=py]
<@\textcolor{red}{func}@> findWays ( N , dp ) :
    if ( N == 0 ) :
        return 1
    if ( dp [ N ] != - 1 ) :
        return dp [ N ]
    cnt = 0
    for i in range ( 1 , 7 ) :
        if ( N - i >= 0 ) :
            cnt = cnt + findWays ( N - i , dp )
    dp [ N ] = cnt
    return dp [ N ]
N = 4
dp = [ - 1 ] * ( N + 1 )
print ( findWays ( N , dp ) )
\end{lstlisting}&
\begin{lstlisting}[style=py]
<@\textcolor{blue}{def}@> findWays ( N , dp ) :
    if ( N == 0 ) :
        return 1
    if ( dp [ N ] != - 1 ) :
        return dp [ N ]
    cnt = 0
    for i in range ( 1 , 7 ) :
        if ( N - i >= 0 ) :
            cnt = cnt + findWays ( N - i , dp )
    dp [ N ] = cnt
    return dp [ N ]
N = 4
dp = [ - 1 ] * ( N + 1 )
print ( findWays ( N , dp ) )
\end{lstlisting}\\
\hline
\end{tabular}
\end{table*}


==> tables_figs_tex/case_study_java_cpp_one.tex <==
\begin{table*}[h!]
% \hskip-0.5cm
\caption{Qualitative comparison for Java-C++ translation between CodeT5 and \modelname. i) CodeT5 generates a non-standard data type \begin{tt}subset\end{tt} without defining it or importing it. \modelname generates the correct datatype. ii) CodeT5 generetes the wrong tokens to return out of a function, \modelname is able to generate the correct C++ syntax.}
\label{tab:java_cpp_qualitative}
\begin{tabular}{|P{5.0cm}|P{5.0cm}|P{5.0cm}|}

\cline{2-3}\multicolumn{1}{c}{}             & \multicolumn{2}{|c|}{\normalsize{\textbf{Translated C++}}}\\
\hline
\normalsize{\textbf{Source Java}} & \normalsize{\textbf{CodeT5}} & \normalsize{\textbf{\modelname}}\\
\hline
\begin{lstlisting}[style=java]
import java . util . * ;
class GFG {
  static void printVector ( ArrayList < Integer > arr ) {
    if ( arr . size ( ) != 1 ) {
      for ( int i = 0 ;
      i < arr . size ( ) ;
      i ++ ) {
        System . out . print ( arr . get ( i ) + " " ) ;
      }
      System . out . println ( ) ;
    }
  }
  static void findWays ( ArrayList < Integer > arr , int i , int n ) {
    if ( n == 0 ) printVector ( arr ) ;
    for ( int j = i ;
    j <= n ;
    j ++ ) {
      arr . add ( j ) ;
      findWays ( arr , j , n - j ) ;
      arr . remove ( arr . size ( ) - 1 ) ;
    }
  }
  public static void main ( String [ ] args ) {
    int n = 4 ;
    ArrayList < Integer > arr = new ArrayList < Integer > ( ) ;
    findWays ( arr , 1 , n ) ;
  }
}
\end{lstlisting} &
\begin{lstlisting}[style=C++]
#include <bits/stdc++.h>
using namespace std ;
void printVector (<@\textcolor{red}{subset < int , int > arr}@>) {
  if ( arr . size ( ) != 1 ) {
    for ( int i = 0 ;
    i < arr . size ( ) ;
    i ++ ) {
      cout << arr [ i ] << "_" ;
    }
    cout << endl ;
  }
}
void findWays ( vector < int > & arr , int i , int n ) {
  if ( n == 0 ) printVector ( arr ) ;
  for ( int j = i ;
  j <= n ;
  j ++ ) {
    arr . push_back ( j ) ;
    findWays ( arr , j , n - j ) ;
    arr . pop_back ( ) ;
  }
}
int main ( ) {
  int n = 4 ;
  vector < int > arr ;
  findWays ( arr , 1 , n ) ;
}
\end{lstlisting}&
\begin{lstlisting}[style=C++]
#include <bits/stdc++.h>
using namespace std ;
void printVector (<@\textcolor{blue}{vector < int > arr}@> ) {
  if ( arr . size ( ) != 1 ) {
    for ( int i = 0 ;
    i < arr . size ( ) ;
    i ++ ) {
      cout << arr [ i ] << "_" ;
    }
    cout << endl ;
  }
}
void findWays ( vector < int > arr , int i , int n ) {
  if ( n == 0 ) printVector ( arr ) ;
  for ( int j = i ;
  j <= n ;
  j ++ ) {
    arr . push_back ( j ) ;
    findWays ( arr , j , n - j ) ;
    arr . pop_back ( ) ;
  }
}
int main ( ) {
  int n = 4 ;
  vector < int > arr ;
  findWays ( arr , 1 , n ) ;
  return 0 ;
}
\end{lstlisting}\\
\hline
\begin{lstlisting}[style=java]
import java . util . * ;
import java . lang . * ;
class GFG {
  static int minimumIncrement ( int arr [ ] , int N ) {
    if ( N % 2 != 0 ) {
      System . out . println ( "-1" ) ;
      System . exit ( 0 ) ;
    }
    int cntEven = 0 ;
    int cntOdd = 0 ;
    for ( int i = 0 ;
    i < N ;
    i ++ ) {
      if ( arr [ i ] % 2 == 0 ) {
        cntEven += 1 ;
      }
    }
    cntOdd = N - cntEven ;
    return Math . abs ( cntEven - cntOdd ) / 2 ;
  }
  public static void main ( String [ ] args ) {
    int arr [ ] = {
      1 , 3 , 4 , 9 };
      int N = arr . length ;
      System . out . println ( minimumIncrement ( arr , N ) ) ;
    }
  }
\end{lstlisting} &
\begin{lstlisting}[style=C++]
#include <bits/stdc++.h>
using namespace std ;
int minimumIncrement ( int arr [ ] , int N ) {
  if ( N % 2 != 0 ) {
    cout << "-1" ;
    <@\textcolor{red}{c exit ( 0 )}@> ;
  }
  int cntEven = 0 ;
  int cntOdd = 0 ;
  for ( int i = 0 ;
  i < N ;
  i ++ ) {
    if ( arr [ i ] % 2 == 0 ) {
      cntEven += 1 ;
    }
  }
  cntOdd = N - cntEven ;
  return abs ( cntEven - cntOdd ) / 2 ;
}
int main ( ) {
  int arr [ ] = {
    1 , 3 , 4 , 9 };
    int N = sizeof ( arr ) / sizeof ( arr [ 0 ] ) ;
    cout << minimumIncrement ( arr , N ) ;
  }

\end{lstlisting}&
\begin{lstlisting}[style=C++]
#include <bits/stdc++.h>
using namespace std ;
int minimumIncrement ( int arr [ ] , int N ) {
  if ( N % 2 != 0 ) {
    cout << "-1" << endl ;
    <@\textcolor{blue}{return 0}@> ;
  }
  int cntEven = 0 ;
  int cntOdd = 0 ;
  for ( int i = 0 ;
  i < N ;
  i ++ ) {
    if ( arr [ i ] % 2 == 0 ) {
      cntEven += 1 ;
    }
  }
  cntOdd = N - cntEven ;
  return abs ( cntEven - cntOdd ) / 2 ;
}
int main ( ) {
  int arr [ ] = {
    1 , 3 , 4 , 9 };
    int N = sizeof ( arr ) / sizeof ( arr [ 0 ] ) ;
    cout << minimumIncrement ( arr , N ) ;
    return 0 ;
  }
\end{lstlisting}\\
\hline
\end{tabular}
\end{table*}


==> tables_figs_tex/compilation_rate_codet5_table.tex <==
\begin{table}[h]
 \aboverulesep=0ex
 \belowrulesep=0ex
 \renewcommand{\arraystretch}{1.0}
\setlength{\tabcolsep}{8.5pt}
% \renewcommand{\arraystretch}{0.9}
\scriptsize
\rmfamily
\centering
% \hskip-0.3cm
\small
\caption{\label{tab:baseline_compilation}Compilation rate of target languages generated using $\dname$ trained CodeT5, without reinforcement learning. Languages after the `-' are the target languages. Both train and test sets are from the filtered data.}

\begin{tabular}{P{2cm}P{0.7cm}P{0.7cm}}

\toprule
\textbf{Lang Pair} & \textbf{train}  & \textbf{test} \\
\midrule
\textbf{Java-C\#} & 70.97 & 73.87 \\
\textbf{PHP-Python} & 78.70 & 78.60 \\
\textbf{C++-Python} & 72.20 & 75.30 \\
\textbf{Java-C} & 41.88 & 42.85 \\

\arrayrulecolor{black}\bottomrule
\end{tabular}

\end{table}

==> tables_figs_tex/completion_variance.tex <==
% \vspace{-0.5em}
\begin{table}[!ht]
\begin{center}
 \aboverulesep=0ex
 \belowrulesep=0ex
 \renewcommand{\arraystretch}{1.0}
\setlength{\tabcolsep}{7.0pt}
\renewcommand{\arraystretch}{1.3}
% \scriptsize
% \rmfamily
\centering
% \hskip-0.3cm
\small
\caption{\label{tab:completion-variance}  \vspace{-1.0em} Evaluation of performance variance on code completion task over five runs.}

{\fontsize{16}{16}\selectfont
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{lccc}
\toprule
Model & $\uparrow$\textit{xMatch} & $\uparrow$\textit{Edit Sim} & $\uparrow$\textit{Comp Rate} \\
\midrule
CodeT5 (220M) & 42.61 $\pm$ 0.05 & 68.54 $\pm$ 0.49 & 52.14 $\pm$ 4.51 \\
% \hline
\modelname + CodeT5 (220M) & \textbf{42.63} $\pm$ 0.03 & \textbf{69.22} $\pm$ 0.16 & \textbf{97.68} $\pm$ 1.04 \\
\arrayrulecolor{black}\bottomrule
\end{tabular}
}
}
\end{center}
% \vspace{-0.5em}
\end{table}

==> tables_figs_tex/trans_comp_results_v2.tex <==
\begin{table*}[!ht]
\caption{\label{tab:rl4cnct_results}
Summary of  performance comparison between \modelname and baselines on XLCoST. 
The column language headers represent the translation target languages. 
% C++, Java, Python, and C\# are languages with larger number of data points as compared to C and PHP. 
The best results are shown in \textbf{bold} font. 
% \vspace{-0.5em}
}
 \aboverulesep=0ex
 \belowrulesep=0ex
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.2}
\large
\centering
\rmfamily
% \hskip-0.3cm
\resizebox{\textwidth}{!}{
\begin{tabular}{ lcccccccccccc}
 \arrayrulecolor{black}
\toprule
% \cline{3-10}
% \cline{11-14}
Model & \multicolumn{2}{c}{C++} &\multicolumn{2}{c}{Java}& \multicolumn{2}{c}{Python} & \multicolumn{2}{c}{C\#} & \multicolumn{2}{c}{PHP} & \multicolumn{2}{c}{C}\\
\cmidrule(r){2-3}
\cmidrule(r){4-5}
\cmidrule(r){6-7}
\cmidrule(r){8-9}
\cmidrule(r){10-11}
\cmidrule(r){12-13}
% \cmidrule(r){15-16}

&\multicolumn{1}{c}{\textit{CodeBLEU}}& \multicolumn{1}{c}{\textit{CompRate}}& \multicolumn{1}{c}{\textit{CodeBLEU}}& \multicolumn{1}{c}{\textit{CompRate}}& \multicolumn{1}{c}{\textit{CodeBLEU}}& \multicolumn{1}{c}{\textit{CompRate}}& \multicolumn{1}{c}{\textit{CodeBLEU}}& \multicolumn{1}{c}{\textit{CompRate}}& \multicolumn{1}{c}{\textit{CodeBLEU}}& \multicolumn{1}{c}{\textit{CompRate}}& \multicolumn{1}{c}{\textit{CodeBLEU}}& \multicolumn{1}{c}{\textit{CompRate}}\\


% \midrule
\hline

    
Naive Copy & 38.68 & 12.82 & 50.39 & 16.38 & 38.93 & 13.26 & 50.83 & 6.16 & 29.88 & 7.77 & 53.83 & 2.56\\
CodeBERT & 45.34 & 23.38 & 51.28 & 27.89 & 45.07 & 27.62 & 57.63 & 11.30 & 46.53 & 14.67 & 23.69 & 12.06 \\
PLBART & 66.03 & 46.42 & 65.23 & 35.67 & 62.93 & 46.66 & 70.61 & 31.29 & 69.05 & 60.85 & 47.24 & 16.36 \\
CodeT5 & 71.92 & 62.46 & 73.18 & 64.73 & \textbf{73.24} & 69.19 & 75.29 & 63.51 & 79.21 & 78.35 & \textbf{71.42} & 42.70 \\
\modelname + CodeT5 & \textbf{72.11} & \textbf{72.38} & \textbf{73.22} & \textbf{86.95} & 72.67 & \textbf{90.81} & \textbf{75.86} & \textbf{76.71} & \textbf{79.96} & \textbf{85.81} & 70.92 & \textbf{48.82} \\
 \arrayrulecolor{black}
 \bottomrule
 % \hline
\end{tabular}}
% \vspace{-0.5em}
\end{table*}

==> tables_figs_tex/xlcost_filtered_table.tex <==
\begin{table}[t]
 \aboverulesep=0ex
 \belowrulesep=0ex
 \renewcommand{\arraystretch}{1.0}
\setlength{\tabcolsep}{8.5pt}
% \renewcommand{\arraystretch}{0.9}
\scriptsize
\rmfamily
\centering
% \hskip-0.3cm
\small
\caption{\label{tab:filterd_splits}$\dname$ dataset statistics after filtering for compilable programs.}

\begin{tabular}{P{2cm}P{0.8cm}P{0.7cm}P{0.7cm}}

\toprule
\textbf{Lang Pair} & \textbf{train} & \textbf{val}   & \textbf{test} \\
\midrule
\textbf{Java-C\#} & 5081 & 262   & 513 \\
\textbf{PHP-Python} & 1785 & 93  & 201 \\
\textbf{C++-Python} & 5325 & 266 & 529 \\
\textbf{Java-C} & 191 & 34 & 28 \\

\arrayrulecolor{black}\bottomrule
\end{tabular}
\end{table}
